On Verifying Designs With Incomplete Specification

Incompleteness of a specification $\mathit{Spec}$ creates two problems. First, an implementation $\mathit{Impl}$ of $\mathit{Spec}$ may have some $\mathit{unwanted}$ properties that $\mathit{Spec}$ does not forbid. Second, $\mathit{Impl}$ may break some $\mathit{desired}$ properties that are not in $\mathit{Spec}$. In either case, $\mathit{Spec}$ fails to expose bugs of $\mathit{Impl}$. In an earlier paper, we addressed the first problem above by a technique called Partial Quantifier Elimination (PQE). In contrast to complete QE, in PQE, one takes out of the scope of quantifiers only a small piece of the formula. We used PQE to generate properties of $\mathit{Impl}$ i.e. those $\mathit{consistent}$ with $\mathit{Impl}$. Generation of an unwanted property means that $\mathit{Impl}$ is buggy. In this paper, we address the second problem above by using PQE to generate false properties i.e those that are $\mathit{inconsistent}$ with $\mathit{Impl}$. Such properties are meant to imitate the missing properties of $\mathit{Spec}$ that are not satisfied by $\mathit{Impl}$ (if any). A false property is generated by modifying a piece of a quantified formula describing 'the truth table' of $\mathit{Impl}$ and taking this piece out of the scope of quantifiers. By modifying different pieces of this formula one can generate a "structurally complete" set of false properties. By generating tests detecting false properties of $\mathit{Impl}$ one produces a high quality test set. We apply our approach to verification of combinational and sequential circuits.

==> s0torage.tex <==
\footnote{ATPG stands for Automatic Test Pattern
Generation.}
----------
Currently, stuck-at fault tests are generated by a
SAT-solver. Although SAT-solving is in its prime whereas PQE-solving
is just starting, the latter has important advantages (in the context
of fault detection) that may come to fruition. First, to build a test,
a SAT-solver essentially checks the equivalence of $N$ and $N^*$
(describing original and faulty circuits).  So, in the worst case, the
formula to be solved is twice the size of $F$. On the other hand, a
PQE-solver operates on $F^*$ that is of the same size as $F$. Second,
a SAT-solver has to add new variables to propagate the faulty value to
an output variable of $N$~\cite{flt_prop}. (Otherwise, a SAT-solver
has a very poor performance.) A PQE-solver does not need new variables
since it carries out fault propagation via the machinery of clause
redundancy~\cite{hvc-14,certif}.  Third, a SAT-solver excites the
fault site by doing a blind search. On the other hand, a PQE-solver is
well-guided via the machinery of clause redundancy mentioned above.
--------
Namely, the operation of a PQE-solver is based on proving
redundancy of clauses that can be resolved with those of formula $G^*$
(taken out of the scope of quantifiers) or with descendants of
$G^*$.
---------
Below, we show how the formula $F^*$ above is built for the
stuck-at-0 fault on the output line of $g$.
----------
(Like using a set of faults covering the
entire circuit increases the quality of a test set detecting those
faults.)
--------
This algorithm also generates tests breaking these
properties.
-------
*) write a section on relation to previous approaches, mention
    the differences from tests detecing faults:
       +) our intention is to generate faulty properties
          (we provide explanation why these tests works so well)
       +) our approach can be extended to abstract formulas
       +) PQE-solver works differently (does not need to introduce
          new variables)
-----------          
Assume that
computing \rch{M,I} is hard. So one does not know if the specification
\abs{P} is complete. Then one can use the approach described in the
previous sections to form a specification that is complete
\ti{structurally} rather than functionally.

We exploit here the same idea of using PQE to compute properties of
$M$ i.e.  \ti{implementation} properties. Let $Q$ be such a property.
If $P_1 \wedge \dots \wedge P_k \not\imp Q$, then the specification
\abs{P} is \ti{incomplete}. If some states of $M$ falsifying $Q$ (and
hence unreachable from $I$-states) should be reachable, then $M$ is
buggy and must be modified. Otherwise, one needs to update \abs{P} by
adding a specification property $P$ to guarantee that $P_1 \wedge
\dots \wedge P_k \wedge P \imp Q$. The simplest way to achieve this
goal is just to add $Q$ to \abs{P}. Using a procedure similar to that
shown in Fig.~\ref{fig:cmpl_set} one can construct a structurally
complete specification.
--------------
\subsection{General remarks}
Here we continue the notation of previous sections.  Let \abs{P} be a
set of properties \s{P(X,Z)_1,\dots,P_k(X,Z)} specifying a
combinational circuit where $X$ and $Z$ are sets of input and output
variables respectively. Let $N(X,Y,Z)$ be an implementation of the
specification \abs{P}. Let $F(X,Y,Z)$ be a formula describing the
functionality of $N$. Proving the correctness of $N$ reduces to
checking if the equivality $P_1 \wedge \dots \wedge P_k \equiv \prob{Y}{F}$ holds.
This comes down to proving two implications
\begin{itemize}
\item $\prob{Y}{F} \imp (P_1 \wedge \dots \wedge P_k)$;
\item $P_1 \wedge \dots \wedge P_k \imp \prob{Y}{F}$.
\end{itemize}

Checking the first implication is straightforward because it reduces
to proving each property $P_i$ true by showing that $F_i \imp P_i$, $i=1,\dots,k$.
Each of $k$ implications reduces to a SAT problem (although it is possible)


As we mentioned in the introduction, in testing, one addresses
functional incompletness of verification by trying to achieve
\ti{structural} completeness. Here we follow a similar idea.
Namely, we generate a set of false properties that is structurally
complete and then use tests breaking these properties to verify
the implementation $N$. Structural completeness is achieved by
generating fake properties probing every piece of $N$.
---------
Assume one of the implications does not hold. Then one of the three cases occurs.
%
\begin{itemize}
\item for some $P_i \in \abs{P}$ it is hard to prove $F \imp P_i$;
\item it is proved that $P_1 \wedge \dots \wedge P_k \not\imp \prob{Y}{F}$;
\item checking if $P_1 \wedge \dots \wedge P_k \imp \prob{Y}{F}$ is too hard.
\end{itemize}
%
The first case above means that implication .  The second condition says that \abs{P} is
proved to be \ti{incomplete}. The last condition means that proving
the completeness of \abs{P} is hard.
--------
\tb{\scriptsize{2}}\> $\Abs{P}{fls} := \emptyset$ \\
--------
If this requirement does not hold, we have a degenerate case of
$G^*$. (Conjoining $F'$ with $G^*$ is like conjoning a formula with a
false assumption.) Then, a non-empty set of clauses $Q(X)$ is implied
by $F^*$.  On one hand, $Q$ is a false property since $F \not\imp Q$.
On the other hand, $Q$ simply excludes some input assignments to
$X$. So breaking this property is trivial: any input falsifying $Q$ is
a counterexample.
------
\vspace{3pt}
\noindent\ti{Stuck-at-1 on the output line of g}. Formula $F^*$
describing $N^*$ can be obtained by replacing $C_1$ and $C_2$ with
clauses $C^*_1 = v_1 \vee v_3$, $C^*_2 = v_2 \vee v_3$ respectively.
A false property $Q$ is obtained by taking $C^*_1$ and $C^*_2$ out of
the scope of quantifiers in \prob{Y}{C^*_1 \wedge C^*_2 \wedge F'}
where $F' = F \setminus \s{C_1,C_2}$.
-----------
\vspace{3pt}
\noindent\ti{Stuck-at-0 on the output line of g}
---------
\subsubsection{Stuck}
\label{sssec:stuck_at_0}
-------
Subsubsection~\ref{sssec:stuck_at_0}
-----
(the reverse direction
  is obviously true i.e. $\tbl \equiv \stbl$ entails $\tbl \imp
  \stbl$)
---------  
Intuitively, tests breaking $Q$ should be of high quality. The reason
is that they are supposed to break a property that is ``almost
true''. Indeed, the proof of Proposition~\ref{prop:fls_prop} shows
that a test breaking $Q$ makes $N$ and $N^*$ produce different
outputs.  The latter is not a trivial task because $N$ and $N^*$ are
almost identical. The fact that stuck-at fault tests are a special
case of tests breaking false properties (see
Section~\ref{sec:stuck_at}) confirms our intution.
--------
$\forall{X}\prob{Y}{\mi{TT}^*}$ holds
----
%
% subsection
%
\subsection{Building false properties by PQE}
\label{ssec:fls_prop}
 Let $N^*(X,Y,Z)$ be a circuit obtained by replacing a
gate $g$ of $N$ with gate $g^*$. (We assume here that $g$ and $g^*$
have the same set of input variables.) Let $G$ and $G^*$ be formulas
specifying gates $g$ and $g^*$ respectively.  Let $F' = F \setminus
G$. (So, $F = G \wedge F'$.) Then formula $F^*$ equal to $G^*
\!\wedge\!F'$ specifies the functionality of $N^*$.

Let $Q(X,Z)$ be a solution to the PQE problem of taking $G^*$ out of
the scope of quantifiers in \prob{Y}{G^* \wedge F'}.  That is
$\prob{Y}{G^* \wedge F'} \equiv Q \wedge \prob{Y}{F'}$. The
proposition below show that $Q$ is a \tb{false property} of $N$ if $N$
and $N^*$ are inequivalent and vice versa.
%
%  Proposition
%
\begin{proposition}
\label{prop:fls_prop}
$N$ and $N^*$ are inequivalent iff $F \not\imp Q$.
\end{proposition}
\begin{proof} 
  \ti{The ``if'' part.}  Let $F \not\imp Q$. Let
  \pnt{p}=(\pnt{x},\pnt{y},\pnt{z}) be an assignment to \V{F} that
  satisfies $F$ and falsifies $Q$ (i.e. \pnt{p} breaks $F \imp
  Q$). Since $F(\pnt{p}) = 1$, the circuit $N$ outputs \pnt{z} for the
  input \pnt{x}. Since $Q(\pnt{x},\pnt{z})=0$, then $Q \wedge
  \prob{Y}{F'}$ = \prob{Y}{G^* \wedge F'} = \prob{Y}{F^*} = 0 under
  assignment (\pnt{x},\pnt{z}). This means that the circuit $N^*$
  cannot produce the output \pnt{z} for the input \pnt{x}.  So $N$ and
  $N'$ have different outputs for \pnt{x}.
  
  \ti{The ``only if'' part.}  Let $N$ and $N^*$ be inequivalent.  Let
  \pnt{x} be an input for which $N$ and $N^*$ produce different
  outputs.  Let \pnt{p}=(\pnt{x},\pnt{y},\pnt{z}) be the assignment
  describing the execution trace in $N$ under the input \pnt{x}. Then
  \pnt{p} satisfies $F$ and hence $F'$.  Assume the contrary, i.e. $F
  \imp Q$. Then $Q(\pnt{x},\pnt{z})=1$. Since \pnt{p} satisfies $F'$,
  then $Q \wedge \prob{Y}{F'}$ =\prob{Y}{G^* \wedge F'}=
  \prob{Y}{F^*}=1 under assignment (\pnt{x},\pnt{z}). The means that
  $N^*$ produces the output \pnt{z} under the input \pnt{x}. Hence $N$
  and $N^*$ output the same assignment under \pnt{x} and we have a
  contradiction.
\end{proof}
-------
\footnote{The fact that $P_i$
  is a property means that an implementation cannot produce an output \pnt{z} for
  an \input{x} if $P_i(\pnt{x},\pnt{z}) = 0$.}
-----  
Let $N(X,Y,Z)$ be a combinational circuit where $X,Y,Z$ are sets of
input, internal and output variables.  Let $F(X,Y,Z)$ be a formula
specifying $N$.
----------
These properties
are generated to extract tests for verifying
$N$.
-----
In general, $N$ and $N^*$ are not functionally equivalent i.e.
$\prob{Y}{F} \not\equiv \prob{Y}{F^*}$.
----------
\prob{\Sup{W}{int}}{F(\Sup{W}{int},\Sup{W}{ext})}
---------
Incompleteness of a specification \ti{Spec} creates two problems.
First, an implementation \ti{Impl} of \ti{Spec} may have some
\ti{unwanted} properties that \ti{Spec} does not ban. Second,
\ti{Impl} may break some \ti{desired} properties that are not in
\ti{Spec}.  In either case, \ti{Spec} fails to expose bugs of
\ti{Impl}.  In testing, the problem of functional incompleteness is
addressed by running a test set that is complete \ti{structurally}
rather than functionally.  This structural completeness is achieved by
generating tests probing every piece of \ti{Impl}. In an earlier
paper, we showed that a similar approach can be applied to addressing
the first problem above. The idea was to use a technique called
Partial Quantifier Elimination (PQE) to generate properties of
\ti{Impl} i.e. properties \ti{consistent} with \ti{Impl}. In contrast
to complete QE, in PQE, one takes out of the scope of quantifiers only
a small piece of the formula.  In this paper, we continue this line of
research. Namely, we show that on can use PQE to generate properties
that are \ti{inconsistent} with \ti{Impl}. An inconsistent property is
generated by modifying a piece of a quantified formula \Sub{\xi}{impl}
describing \ti{Impl} and taking this piece out of the scope of
quantifiers.  By modifying different piece of \Sub{\xi}{impl} one
can generate a structurally complete set of inconsistent properties.
By generating tests detecting inconsistent properteis of \ti{Impl}
one produces a high quality test. We apply our approach to combinational
and sequential circuits.

